Non-linear Attributed Graph Clustering by Symmetric NMF with PU Learning

We consider the clustering problem of attributed graphs. Our challenge is how we can design an effective and efficient clustering method that precisely captures the hidden relationship between the topology and the attributes in real-world graphs. We propose Non-linear Attributed Graph Clustering by Symmetric Non-negative Matrix Factorization with Positive Unlabeled Learning. The features of our method are three holds. 1) it learns a non-linear projection function between the different cluster assignments of the topology and the attributes of graphs so as to capture the complicated relationship between the topology and the attributes in real-world graphs, 2) it leverages the positive unlabeled learning to take the effect of partially observed positive edges into the cluster assignment, and 3) it achieves efficient computational complexity, $O((n^2+mn)kt)$, where $n$ is the vertex size, $m$ is the attribute size, $k$ is the number of clusters, and $t$ is the number of iterations for learning the cluster assignment. We conducted experiments extensively for various clustering methods with various real datasets to validate that our method outperforms the former clustering methods regarding the clustering quality.

==> 11_aaai_inproc.tex <==

%% graph clustering 
@article{karypis1998multilevelk,
  title={Multilevelk-way partitioning scheme for irregular graphs},
  author={Karypis, George and Kumar, Vipin},
  journal={Journal of Parallel and Distributed computing},
  volume={48},
  number={1},
  pages={96--129},
  year={1998},
  publisher={Elsevier}
}

@inproceedings{ben1999clustering,
  title={Clustering gene expression patterns},
  author={Ben-Dor, Amir and Yakhini, Zohar},
  booktitle={Proceeding of\ RECOMB},
  pages={33--42},
  year={1999},
}

@article{flake2002self,
  title={Self-organization and identification of web communities},
  author={Flake, Gary William and Lawrence, Steve and Giles, C Lee and Coetzee, Frans M},
  journal={Computer},
  volume={35},
  number={3},
  pages={66--70},
  year={2002},
  publisher={IEEE}
}

@article{brohee2006evaluation,
  title={Evaluation of clustering algorithms for protein-protein interaction networks},
  author={Brohee, Sylvain and Van Helden, Jacques},
  journal={BMC bioinformatics},
  volume={7},
  number={1},
  pages={488},
  year={2006},
  publisher={BioMed Central}
}

@article{newman2006modularity,
  title={Modularity and community structure in networks},
  author={Newman, Mark EJ},
  journal={Proceedings of the national academy of sciences},
  volume={103},
  number={23},
  pages={8577--8582},
  year={2006},
  publisher={National Acad Sciences}
}
@article{karrer2010dcsbm,
  title={Stochastic blockmodels and community structure in networks},
  author={Karrer, Brian and Newman, M., E., J. },
  journal={Physical Review},
  year={2011},
  number={E 83}
%   volume={103},
%   pages={8577--8582},
%   publisher={}
}

@article{yan2014degree,
  title={Model Selection for Degree-corrected Block Models},
  author={Yan,Xiaoran and Shalizi, Cosma, Rohilla, and Jensen, Jacob E.and Krzakala, Florent and Moore, Cristopher and Zdeborova, Lenka and Zhang, Pan and Zhu, Yaojia},
  journal={Journal of Statistical Mechanics},
  year={2014},
  number={P05007}
%   pages={8577--8582},
%   publisher={}
}

@inproceedings{xu2007scan,
  title={Scan: a structural clustering algorithm for networks},
  author={Xu, Xiaowei and Yuruk, Nurcan and Feng, Zhidan and Schweiger, Thomas AJ},
  booktitle={Proceeding of\ SIGKDD},
  year={2007},
}

@inproceedings{zhou2009saclus,
  title={Clustering large attributed graphs: an efficient
incremental approach},
  author={Zhou, Yang and Cheng, Hong and Yu, Jeffrey, Xu},
  pages={689--698},
  year={2010},
  booktitle={Proceeding of\ ICDM}
}

@inproceedings{zhou2010incclus,
  title={Graph clustering based on structural/attribute similarities},
  author={Zhou, Yang and Cheng, Hong and Yu, Jeffrey, Xu},
  pages={718--729},
  year={2009},
  booktitle={Proceeding of\ VLDB}
}

@article{kulis2009semi,
  title={Semi-supervised graph clustering: a kernel approach},
  author={Kulis, Brian and Basu, Sugato and Dhillon, Inderjit and Mooney, Raymond},
  journal={Machine learning},
  volume={74},
  number={1},
  pages={1--22},
  year={2009},
  publisher={Springer}
}

@article{fortunato2010community,
  title={Community detection in graphs},
  author={Fortunato, Santo},
  journal={Physics reports},
  volume={486},
  number={3-5},
  pages={75--174},
  year={2010},
  publisher={Elsevier}
}
@inproceedings{xu2012model,
  title={A model-based approach to attributed graph clustering},
  author={Xu, Zhiqiang and Ke, Yiping and Wang, Yi and Cheng, Hong and Cheng, James},
  booktitle={Proceeding of\ SIGMOD},
  year={2012},
}

%graph database
@article{Sahu2017ubiquity,
  author    = {Siddhartha Sahu and
               Amine Mhedhbi and
               Semih Salihoglu and
               Jimmy Lin and
               M. Tamer {\"{O}}zsu},
  title     = {The Ubiquity of Large Graphs and Surprising Challenges of Graph Processing},
  journal   = {{PVLDB}},
  volume    = {11},
  number    = {4},
  pages     = {420--431},
  year      = {2017}
}

@inproceedings{Francis2018Cypher,
 author = {Francis, Nadime and Green, Alastair and Guagliardo, Paolo and Libkin, Leonid and Lindaaker, Tobias and Marsault, Victor and Plantikow, Stefan and Rydberg, Mats and Selmer, Petra and Taylor, Andr{\'e}s},
 title = {Cypher: An Evolving Query Language for Property Graphs},
 booktitle = {SIGMOD},
 year = {2018}
} 

@misc{oracle,
 author = {Oracle}
 title = {Oracle Spatial and Graph},
 howpublished = {http://www.oracle.com/us/products/database/options/spatial/overview/index.html}
 }

%% Matrix factorization
@inproceedings{ding2006orthogonal,
  title={Orthogonal nonnegative matrix t-factorizations for clustering},
  author={Ding, Chris and Li, Tao and Peng, Wei and Park, Haesun},
  booktitle={Proceeding of\ SIGKDD},
  year={2006},
}

@inproceedings{kuang2012symmetric,
  title={Symmetric nonnegative matrix factorization for graph clustering},
  author={Kuang, Da and Ding, Chris and Park, Haesun},
  booktitle={Proceeding of\ SDM},
  year={2012},
}

@inproceedings{hsieh2015pu,
  title={PU Learning for Matrix Completion.},
  author={Hsieh, Cho-Jui and Natarajan, Nagarajan and Dhillon, Inderjit S},
  booktitle={Proceeding of\ ICML},
  year={2015}
}

@inproceedings{huang2017joint,
  title={Joint weighted nonnegative matrix factorization for mining attributed graphs},
  author={Huang, Zhichao and Ye, Yunming and Li, Xutao and Liu, Feng and Chen, Huajie},
  booktitle={Proceeding of\ PAKDD},
  year={2017},
}


@article{lee1999learning,
  title={Learning the parts of objects by non-negative matrix factorization},
  author={Lee, Daniel D and Seung, H Sebastian},
  journal={Nature},
  volume={401},
  number={6755},
  pages={788},
  year={1999},
}

@article{kuang2015symnmf,
  title={SymNMF: nonnegative low-rank approximation of a similarity matrix for graph clustering},
  author={Kuang, Da and Yun, Sangwoon and Park, Haesun},
  journal={Journal of Global Optimization},
  volume={62},
  number={3},
  pages={545--574},
  year={2015},
  publisher={Springer}
}

@inproceedings{aleksandar2018paican,
  title={Bayesian Robust Attributed Graph Clustering: Joint Learning of Partial Anomalies and Group Structure},
  author={Aleksandar, Bojchevski and Stephan, Günnemann}, 
  booktitle={Proceeding of AAAI},
  pages={2738--2745},
  year={2018},
}

@inproceedings{kipf2017semi,
  title={Semi-Supervised Classification with Graph Convolutional Networks},
  author={Kipf, Thomas N. and Welling, Max},
  booktitle={Proceeding of\ ICLR},
  year={2017}
}

==> table/ari_long.tex <==

\begin{small}
\begin{table*}[t]\setlength{\tabcolsep}{5pt}
  \caption{The average and standard deviation (in parenthesis) of ARI. The methods annotated with * indicate the parameters are initialized by random values. 
  The boldface font represents the best performance for each dataset.}
  \label{tb: ari}
  \setlength{\tabcolsep}{5pt}
  \begin{center}
	\begin{tabular}{|l|c|c|c|c|} \hline
        Method & WebKB & Citeseer & Cora  &  polblog \\ \hline \hline
        Prop. & ${\bf 0.995} ~{(\pm 0.002)}$ &$ {\bf 0.280} ~{(\pm 0.027)} $& ${\bf 0.348} ~{(\pm 0.022)}$ &${\bf 0.626} ~{(\pm 0.037)}$\\ \hline
        Prop. (w/o PU)&$0.990~{(\pm 0.005)}$&$0.221~{(\pm 0.010)}$&$0.270~{(\pm 0.024)}$&$0.621~{(\pm 0.000)}$\\ \hline
        Prop. $^{*}$& $ 0.982~{(\pm 0.003)}$ & $ 0.126 ~{(\pm 0.023)}$ & $0.244 ~{(\pm 0.038)}$ &  $ 0.603 ~{(\pm 0.011)}$\\ \hline
        JWNMF  & $0.906 ~{(\pm 0.000)}$ & $0.127 ~{(\pm 0.000)}$ & $0.230 ~{(\pm 0.000)}$ & $0.517 ~{(\pm 0.000)}$ \\ \hline
        JWNMF$^{*}$ & $0.909 ~{(\pm 0.002)}$ &$ 0.082 ~{(\pm 0.009)}$ & $ 0.227 ~{(\pm 0.011)}$ & $0.504 ~{(\pm 0.011)}$\\ \hline
        BAGC & $0.204 ~{(\pm 0.000)}$ & $0.000 ~{(\pm 0.000)}$ & $0.016 ~{(\pm 0.000)}$ & $0.000 ~{(\pm 0.000)}$\\ \hline
        SNMF & $0.840 ~{(\pm 0.100)}$ &$ 0.067 ~{(\pm 0.020)}$ & $0.211 ~{(\pm 0.023)}$ &  $0.498 ~{(\pm 0.059)}$ \\ \hline
        NMF & $0.327 ~{(\pm 0.004)}$ & $0.193 ~{(\pm 0.023)}$ & $0.115 ~{(\pm 0.001)}$ & $0.000 ~{(\pm 0.000)}$  \\ \hline
        k-means & $0.260 ~{(\pm 0.131)}$ &$  0.190 ~{(\pm 0.044)}$ & $0.093 ~{(\pm 0.034)}$ & $0.000 ~{(\pm 0.000)}$\\ \hline 
        METIS & $0.851 ~{(\pm 0.000)}$ & $0.156 ~{(\pm 0.000)}$ & $0.283 ~{(\pm 0.000)}$ & $0.545 ~{(\pm 0.000)}$\\ \hline 
 	\end{tabular}
 \end{center}
\end{table*}
\end{small}
